Stable Approximation Algorithms for Dominating Set and Independent Set

We study the Dominating set problem and Independent Set Problem for dynamic graphs in the vertex-arrival model. We say that a dynamic algorithm for one of these problems is $k$-stable when it makes at most $k$ changes to its output independent set or dominating set upon the arrival of each vertex. We study trade-offs between the stability parameter $k$ of the algorithm and the approximation ratio it achieves. We obtain the following results. 1. We show that there is a constant $\varepsilon^*>0$ such that any dynamic $(1+\varepsilon^*)$-approximation algorithm the for Dominating set problem has stability parameter $\Omega(n)$, even for bipartite graphs of maximum degree 4. 2. We present algorithms with very small stability parameters for the Dominating set problem in the setting where the arrival degree of each vertex is upper bounded by $d$. In particular, we give a $1$-stable $(d+1)^2$-approximation algorithm, a $3$-stable $(9d/2)$-approximation algorithm, and an $O(d)$-stable $O(1)$-approximation algorithm. 3. We show that there is a constant $\varepsilon^*>0$ such that any dynamic $(1+\varepsilon^*)$-approximation algorithm for the Independent Set Problem has stability parameter $\Omega(n)$, even for bipartite graphs of maximum degree $3$. 4. Finally, we present a $2$-stable $O(d)$-approximation algorithm for the Independent Set Problem, in the setting where the average degree of the graph is upper bounded by some constant $d$ at all times. We extend this latter algorithm to the fully dynamic model where vertices can also be deleted, achieving a $6$-stable $O(d)$-approximation algorithm.

==> Additive_No_SAS.tex <==
\section{Non existence of additive approximation of the maximum independent set in trees}

One might guess that in the dynamic model if all the graphs that are formed over time are relatively simple for example if they belong to the class of trees or forest it might be possible to get an additive approximation of the maximum independent set with a bounded stability parameter. By additive approximation we mean to say that there exists a absolute constant $c$ and an algorithm \alg with a bounded stability parameter $k_c$ such that \alg that maintains an independent set of size greater than or equal to $\opt-c$ at all times. In this section we show that such an additive approximation does not exist even when the dynamic graphs formed are are trees.

==> Bounded_approximation_Algorithms_with_bounded_stability_for_bounded_degree_arrival_model.tex <==
\section{Bounded approximation algorithm with bounded stability parameter in a special case of the online arrival model}

\subsection{Maximum Independent Set}

In this section we consider the online arrival model where at every instance a vertex arrives along with some edges adjacent to the already existing graph. We also restrict our model to the case where all the intermediate sequence of graphs $G_0=\{v\}, G_1, G_2, G_3, \ldots $ formed in the online arrival model has a average degree bounded by a constant $d$. In the previous section we see that it is not possible to get an approximation factor close to $1$ even with arbitrarily large stability parameter. Also it is easy to observe that in this model if we allow just one change after each arrival of vertex it's not possible to get a bounded approximation ratio but in this section we show that it is possible to get a bounded approximation ratio with only $2$ changes after each arrival of a vertex. 

\begin{theorem}
There exists a $2$-stable algorithm that achieves an approximation ratio of $d^2$.

\end{theorem}

\begin{proof}
Let $G$ be a 



\end{proof}

\subsection{Minimum Dominating Set}
In this section we prove that a 1-stable $d^2$ approximation algorithm exists for the online minimum dominating set problem where at every instance a vertex arrives with degree at most $(d+1)^2$.

The algorithm is based on the following two ideas.
\begin{itemize}
    \item 

Let $\opt_{out}$ denote the minimum size of a dominating set under the condition that every node should be dominated by itself or by an out-neighbor (if we direct edges from the younger nodes to the older nodes, that is, a node arrives with all its outgoing edges). Let $\opt$ be be minimum size of a dominating set without this restriction. Then we can show $\opt_{out} \leq (d+1) \opt$.  (Proof: Take an unrestricted dominating set. Then the union of that set plus all their out-neighbors is a restricted dominating set.)
\item Let $N^+[v] := \{v\} \cup \{\text{out-neighbors of v}\}$. Call two nodes $u,v$ unrelated if $N^+[v] \cap N^+[u] = \emptyset$. Note that this implies that $u$ and $v$ must be dominated by different nodes in $\opt_{out}$. Thus, if $U$ is a set of pairwise unrelated nodes, then $\opt_{out} \geq |U|$.

\end{itemize}

The algorithm is now as follows. We initialize $D := \emptyset$ (D will be our dominating set) and $U := \emptyset$. We maintain the following invariants:
\begin{itemize}
    \item 

\item $U$ is a set of pairwise unrelated nodes
\item All nodes in $D$ are an out-neighbor of a node in $U$ or are in $U$ themselves.
\end{itemize}
Hence. $|D| \leq (d+1) |U| \leq (d+1) \opt_out \leq (d+1)^2 \opt$.
Here's the algorithm to process $v$:
Case I: $N^+[v] \cap D \neq \emptyset$.
In other words, one of the out-neighbors of $v$ is already in  our dominating set. In this case we do nothing.
Case 2: $N^+[v] \cap D = \emptyset$ and $v$ is unrelated to all nodes $u\in U$
We now add $v$ to $U$, and we pick an arbitrary node $w \in N^+[v]$ and add $w$ to $D$. (So we might as well pick $w=v$.)
Case 2: $N^+[v] \cap D = \emptyset$ and there is a node $u \in U$ that is related to $v$.
We now pick an arbitrary node $w \in N^+[u] \cap N^+[v]$, and add $w$ to $D$. ($U$ is unchanged.)
Note that the invariants are maintained in all cases.

Below we show that the approximation ratio $\Theta(d^2)$ is tight for this algorithm.


\subsection*{3-stable Algorithm with approximation ratio $O(d)$}

In this section we describe a $3$ stable $4.5d$ approximation algorithm for the online dominating set problem with each arriving vertex arrives with degree at most $d$ at every instance. The algorithm works in two phases.


\begin{algorithm}[H] 
\caption{\textsc{Achieve Target}$(D(t),\opt)$}
\begin{algorithmic}[1]
%
\State $\rhd$ Let $r_k=|J_k|/|I_k|$
\If{$|I_k|+|J_k| \leq k_\eps$}
\State $J^*=J_k$ and output $J^*$.
\Else

    
      \State Find a balanced separator $S_k$ of $G_k$ that separates the graph into two parts $A$ and $B$. Let $I_k \cap A=I_{k,A}$, $J_k \cap A=J_{k,A}$,  $I_k \cap B=I_{k,B}$,  $J_k \cap B=J_{k,B},  I_k \cap S_k=I_{k,S_k},  J_k \cap S_k=J_{k,S_k}$. 
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} < min(1+\eps, r_k)$ and $\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} < min(1+\eps, r_k)$} 
      \State  \textsc{Separate and Iterate}$(G^A,k_\eps)$ where $G^A$ is the induced bipartite subgraph of $G$ with vertices $J_{k,A} \cup I_{k,A} \cup I_{k,S_k}$. 
      \EndIf
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} \geq min(1+\eps, r_k)$}
      \State \textsc{Separate and Iterate}$(G^A,k_\eps)$
        \EndIf
      \If{$\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} \geq min(1+\eps, r_k)$}
      \State \textsc{Separate and Iterate}$(G^B,k_\eps)$ where $G^B$ be the induced bipartite subgraph of $G$ with vertices $J_{k,B} \cup I_{k,B} \cup I_{k,S_k}$.
     
      
      \EndIf
\EndIf
\end{algorithmic}
\end{algorithm}





We describe the algorithm below:

\begin{itemize}
    \item We denote $D(t)$ to be the output dominating set at time $t$. Initialize $D(1)=v_1$ after arrival of the first vertex at time $1$.

    \item 
\end{itemize}







==> No_SAS_in_Expanders.tex <==
\section{No SAS in a sequence of expanders graphs with bounded degree}
%------------------------------------------------------------------------------------------
\subsection{No SAS for Maximum Independent Set}
In this section we will create a sequence of graphs $\{G_t\}$ which somewhat behaves like a vertex expander for which we prove that no SAS exists. Before we move to our construction we give a few definitions. 
%------------------------------------------------------------------------------------------
\begin{flushleft}
\begin{definition}
For any subset $S$ of vertices of a graph $G=(V,E)$, define the neighbourhood $N(S)=\{u| \exists v\in S\ \text{such that}\ (u,v)\in E\}$.
\end{definition}

\begin{definition}
A graph $G=(V,E)$ is a $(K,A)$ vertex expander if for all sets $S$ of at most $K$ vertices, the neighbourhood $N(S)$ is of size at least $A\cdot|S|$.
\end{definition}

\begin{definition}
A double cover of a graph $G=(V,E)$ is a bipartite graph $\tilde{\tilde{G}}$ which has two vertices $u_i$ and $w_i$ for each vertex $v_i$ of $G$ and two vertices $u_i$ and $w_j$ of $\tilde{\tilde{G}}$ are connected by an edge if and only if $v_i$ and $v_j$ are connected by an edge in $G$.
\end{definition}
\end{flushleft}
%------------------------------------------------------------------------------------------

\begin{theorem} \label{thm:expander existence}
For all constants $D \geq 3$, there is a constant $0<\alpha<1$ such that for all $n$, a random $D$-regular undirected graph on $n$ vertices is an $(\alpha n, D-1.01)$ vertex expander with probability at least $1/2$.
\end{theorem}
\begin{proof}
Refer to Expander pdf.
\end{proof}

In particular theorem \ref{thm:expander existence} shows the existence of a $3$-regular graph $G'$ which is a $(\alpha n, 1.99)$ vertex expander. Call $H'=L' \cup R'$ be the bipartite double cover of $G'$. Let $L'=\{l_1, l_2, \ldots , l_n\}$ and let $\{e_{i,1}, e_{i,2}, \ldots , e_{i,j_i}\}$ be the corresponding edges adjacent to $l_i$. 

\begin{lemma} \label{thm:property of bipartite expander}
For all sets $S\subseteq L'$ of at most $\alpha n$ vertices, $N(S)\subseteq R'$ has size at least $1.99\cdot|S|$.
\end{lemma}
\begin{proof}
Trivial.
\end{proof} 

\begin{flushleft}

 Let $\eps:=\min \left(\frac{\alpha}{384-\alpha}, \frac{2-\alpha}{16+\alpha}\right)$. We suppose there exists an $\alg$ that maintains an approximation ratio of $1+\eps$ and has a stability parameter bounded by $k_{\eps}$. Choose a natural number $n$ such that $k_{\eps} \leq \frac{1}{384}\lfloor{\alpha n}\rfloor$.
 \arp{This is the only condition on $k_\eps$ we need for the proof to work and which is still true in the case when $k_\eps$ depends on also n and equals $o(n)$, just choose $n$ large enough} Now we construct a graph $G$ in an online manner. Let $G_t$ be the online graph formed after arrival of the $t^{th}$ vertex. Let $I_{\alg_t}$ be the set of vertices in the output independent set of $\alg$ after arrival of the $t^{th}$ vertex. Also let $I_t$ be the set of vertices in a maximum independent set of $G_t$. We will show the impossibility of existence of SAS using the construction of a series of insertions below which is inspired from the bipartite double cover $H'$. \newline

\emph{Construction of the graph $G$ in an online manner:} 

\begin{itemize}
    \item First $|R'|=n$ number of isolated vertices arrive one by one. 
    \item Next the vertices $l_i$, $i=\{1, 2, \ldots, n\}$ along with their corresponding edges $\{e_{i,1}, e_{i,2}, \ldots , e_{i,j_i}\}$ arrives one by one.
    \item Then $\lfloor{\frac{n}{4}}\rfloor$ number of new degree $3$ vertices arrive one by one and each of them connected to distinct $3$ vertices in $R'$. We denote this set of vertices by $S$.
\end{itemize}

Observe that after $2n$ steps we have a realisation of the graph $H'$ which is formed in an online manner. Then a few more degree $3$ vertices arrive that have edges adjacent to $R'$. Also note that it is possible to construct in a way such that no two vertices in $S$ share a common neighbour as cardinality of $S$ is strictly less than $n/3$. Observe that the degree of every vertex of the online graph is less than or equal to $4$ at all instance.

\begin{lemma} \label{thm:property of construction}
If the approximation ratio is bounded by $1+\eps$ then the number of vertices in $I_{\alg_t} \cap (L' \cup S)$ is strictly less than $\frac{\alpha n}{16}$ for all $t=n+1, n+2, n+3, \ldots , 2n+ \lfloor{\frac{n}{4}}\rfloor$.
\end{lemma}
\begin{proof}
For the sake of contradiction assume $t_f$ to be the first time in which $|I_{\alg_{t_f}} \cap (L' \cup S)| \geq \frac{\alpha n}{16}$. Clearly as the stability parameter of $\alg$ is equal to $k_\eps$, we have that at time $t_f$, $|I_{\alg_{t_f}} \cap (L' \cup S)| \leq \frac{\alpha n}{16} + k_\eps$. Let $I_{\alg_{t_f}} \cap L'=V_1$ and $I_{\alg_{t_f}} \cap S=V_2$. We do the following case distinction

\emph{Case 1:} If $|V_1| \geq \frac{7}{12} \times \frac{\alpha n}{16}$, then by  theorem \ref{thm:property of bipartite expander} we have $N(V_1)>\frac{13}{12} \times \frac{\alpha n}{16}$. Hence cardinality of $|I_{\alg_{t_f}} \cap R'| \leq n-\frac{13}{12} \times \frac{\alpha n}{16}$. Hence $|I_{\alg_{t_f}}|=|I_{\alg_{t_f}} \cap R'| + |I_{\alg_{t_f}} \cap (L' \cup S)| \leq  \frac{\alpha n}{16} + k_\eps + n-\frac{13}{12} \times \frac{\alpha n}{16} =k_\eps + n-\frac{1}{12} \times \frac{\alpha n}{16} <n- \frac{\alpha n}{384}$. Hence the approximation ratio maintained by $\alg$ at time $t_f$ is strictly greater than $\frac{n}{n- \frac{\alpha n}{384}}=1+\frac{\alpha}{384-\alpha} \geq 1+\eps$ which is a contradiction.

\emph{Case 2:} If $|V_1| < \frac{7}{12} \times \frac{\alpha n}{16}$, then we have $|V_2| \geq \frac{5}{12} \times \frac{\alpha n}{16}$. So by construction we have $N(V_2)>\frac{15}{12} \times \frac{\alpha n}{16}$. Hence cardinality of $|I_{\alg_{t_f}} \cap R'| \leq n-\frac{15}{12} \times \frac{\alpha n}{16}$. Hence $|I_{\alg_{t_f}}|=|I_{\alg_{t_f}} \cap R'| + |I_{\alg_{t_f}} \cap (L' \cup S)|$ and now $|I_{\alg_{t_f}} \cap R'|$ is even lesser than in \emph{Case 1}, so we have that the approximation ratio maintained by $\alg$ at time $t_f$ is strictly greater than $1+\eps$ which is again a contradiction.

Hence we have our theorem.
\end{proof}

\begin{theorem}
$\alg$ cannot maintain an approximation ratio of $1+\eps$. Hence we have no SAS for the online arrival model in which all vertices of the online graph has degree less than or equal to $4$ at all times.
\end{theorem}
\begin{proof}
Let $t=2n+ \lfloor{\frac{n}{4}}\rfloor$, then by lemma \ref{thm:property of construction} we have $|I_{\alg_t} \cap (L' \cup S)| \leq \frac{\alpha n}{16}$, also $|I_{\alg_t} \cap R'| \leq n$. So we have $|I_{\alg_{t}}|=|I_{\alg_{t}} \cap R'| + |I_{\alg_{t}} \cap (L' \cup S)| \leq n+ \frac{\alpha n}{16}$. Hence the approximation ratio $\frac{I_t}{I_{\alg_t}} > \frac{n+n/8}{n+ \alpha n/16}=\frac{18}{16+\alpha}=1+\frac{2-\alpha}{16+\alpha} \geq 1+\eps$ which is a contradiction.
\end{proof}

-

\end{flushleft}

\subsection{No SAS for Minimum Dominating Set}

In this section we prove that No SAS exists for the minimal dominating sets. We will use the definitions of the previous section. 

\begin{lemma} \label{thm:property of special bipartite expander }
For all natural number n large enough there exists a bipartite graph $H= (L \cup R)$ with $|L|=\lceil{(1-\frac{1}{21})n}\rceil$ and $|R|=n$ such that the following holds:
\begin{itemize}
    \item the degree of each vertex is greater than $4$ and less than $5$.
    \item  each vertex in $R$ is adjacent to some vertex of $L$.  
    \item there exists a constant $\alpha<1$ such that for any $S\subseteq L$ of at most $\alpha n$ vertices, $N(S)\subseteq R$ has size at least $3.99\cdot|S|$.

\end{itemize}
\end{lemma}
\begin{proof}
Follows from \ref{thm:expander existence} after deleting some selected vertices(So that no vertex of $R$ is left isolated) from the double cover of the expander in \ref{thm:expander existence}. Since we are only deleting vertices the expansion property (from left to right) isn't affected. (Needs to be carefully checked).
\end{proof} 

\emph{Construction of the graph $G$ in an online manner:} 

\begin{itemize}
    \item First a set $F'$ of $5n$ isolated vertices arrive one by one. Divide them into $n$ groups of $5$ vertices namely $F_1, F_2, \ldots F_n$. In each group $F_i$ fix some ordering of the $5$ vertices. Let $F_i= \{v_{1_i}, v_{2_i}, v_{3_i}, v_{4_i}, v_{5_i}\}$. Call $F=\{ F_1, F_2, F_3, \ldots, F_n\}$, where $F_i$ is the $i^{th}$ flower.
    \item Next $n$ vertices $E=\{v_1, v_2, v_3, \ldots, v_n$\} arrive one by one with each having degree exactly equal to $5$. The vertex $v_i$ is adjacent to all vertices of $F_i$ for all $i=1, 2, 3,\ldots , n$.
    \item Then a set $D$ with $|D|=\lceil{(1-\frac{1}{21})n}\rceil$ number of new vertices arrive along with their edges such that:
    \begin{itemize}
        \item the bipartite graph formed with vertices $D \cup F$ is isomorphic to $H=L \cup R$ (here $H$ is the bipartite expander in \ref{thm:property of special bipartite expander } and $D=L$ and $F=R$ (Needs more proper writing)). Note that here we are treating the flowers $F_i's$ consisting of $5$ vertices as a single vertex of the bipartite expander graph isomorphic to $H$ and using the convention that if a vertex $d_i \in D$ has an edge to at least one vertex of the flower $F_j$ then $d_i$ and $F_j$ has an edge. We call such an edge between a flower and a vertex of $D$ a "large" edge.
        
        \item Each vertex $d_i$ of $D$ is adjacent to exactly $2$ vertices of $E$ with the only condition that all vertices of $E$ are adjacent to some vertex of $D$.
        
        \item We know that each flower $F_i$ is adjacent to at most $5$ but at least $4$ vertices of $D$. Now during the process of arrival of vertices of $D$, the first vertex of $D$ to hit $F_i$ is adjacent to $v_{1_i}$ and $v_{2_i}$, the second vertex of $D$ to hit $F_i$ is adjacent to $v_{3_i}$ and $v_{4_i}$, the third vertex of $D$ to hit $F_i$ is adjacent to $v_{1_i}$ and $v_{5_i}$, the fourth vertex of $D$ to hit $F_i$ is adjacent to $v_{2_i}$ and $v_{4_i}$, the fifth vertex of $D$ to hit $F_i$(if it exists) is adjacent to $v_{3_i}$ and $v_{5_i}$.
    \end{itemize}
\end{itemize}

Let $\eps:=\min \left(1.04, 1+0.3\alpha \right)$. And suppose there exists a SAS for minimal dominating set problem. So assume $k_\eps$ to be the stability parameter sufficient to maintain an approximation ratio of $\eps:=\min \left(1.04, 1+0.3\alpha \right)$. Call a flower $F_i$ to be fully dominated by a set $S$ if all vertices in $F_i$ is adjacent to some vertex of $S$. Let $ODS$ be the output dominating set (not a good notation as we need to specify time but i keep it for now).

\begin{observation}\label{obs:Observations about the Construction}

\begin{itemize}
    \item Any $4$ "large" edge from $D$ to a flower $F_i$ is sufficient to fully dominate $F_i$(convinced?). Hence by construction we know that all $5n$ vertices of the set $F'$ is adjacent to some vertex of $D$. So the set $D$ fully dominates $F'$.
    
      \item The set $D$ also fully dominates $E$.
    
    \item At least $3$ "large" edge from $D$ to a flower $F_i$ is necessary to fully dominate $F_i$.
    
    \item The size of the minimal dominating set is less than or equal to $n$ after arrival of all the vertices of $E$ till the end of the construction.
    
    \item The size of the minimal dominating set is less than or equal to $(1-\frac{1}{21})n$ at the end of the construction.
    
  
\end{itemize}



\end{observation}

\begin{proof}
I think the first point is not necessary but i still keep it for now. Directly from construction we can see that $D$ fully dominates the $5n$ vertices of $F'$. The proofs of the rest of the observations are trivial.
\end{proof}

\begin{lemma}
Suppose at any time point $ODS$ be the output dominating set. Let $S=ODS \cap D$. Suppose $S$ fully dominates exactly $f$ flowers then $|ODS| \geq n-f+|S|$.
\end{lemma}
\begin{proof} Idea:
There exists vertices that are not dominated by $S$ in exactly $n-f$ distinct flowers. And each such vertex from a distinct flower will force one new vertex in the ODS which does not belong to $D$. Hence the result.  
\end{proof}

\begin{lemma}
Suppose at any time point $|ODS \cap D| \leq \alpha n$. Then $|ODS| \geq n$. Hence if we maintain an approximation ratio of $\eps$ then at the end of the construction $ODS \cap D$ must be greater than $\alpha n$.
\end{lemma}
\begin{proof}
Idea: Let $S=ODS \cap D$ and let $|S| \leq \alpha n$. We know that for $S$ to fully dominate a flower $F_i$ we need at least $3$ "large" edges from $S$ to $F_i$. So if $f$ is the number of fully dominated flowers by $S$ then we have already used up $3f$ large edges. The remaining number of large edges is at most $5|S|-3f$ (As each vertex in $D$ has at most $5$ large edges attached to it due to the degree constraint of the expander). We also know that the number of distinct flowers hit by $S$ is at least $3.99|S|$ (due to construction and the expansion factor of the expander). So we know $3.99|S| \leq 5|S|-3f +f$ hence $f \leq 0.505|S|$ ($5|S|-3f +f$ is the maximum number of distinct flowers hit by S). So putting the inequality of $f$ in the previous lemma we get $|ODS| \geq n$. Hence we have our theorem as in the end it would create a problem because of the desired approximation ratio that we want to maintain.
\end{proof}


So far we managed to proof that by the end of the construction any output dominating set that wants to maintain an $1+\eps$ approximation with $\opt$ must have at least $\alpha n$ vertices from $D$. Next we show that even that creates a problem.

\begin{lemma}
Suppose $t_f$ be the first time point when $ODS \cap D> \alpha n$. Then $|ODS| \geq n+0.4\alpha$. Hence we cannot maintain an approximation ratio of $1+\eps$ at time $t_f$. Therefore it is not possible to have a SAS.
\end{lemma}
\begin{proof}
Idea: Again let $S=ODS \cap D$ . Very similar proof to the previous lemma. We know at time $t_f$, $\alpha n<|S| \leq \alpha n+ k_\eps$, now $k_\eps$ can be made very small w.r.t $\alpha n$ so that won't create any problem and so you can assume that |S| is almost exactly equal to $\alpha n$. The difference in proof from the previous lemma is that here we have $|S| \geq \alpha n$. We have the same set of inequalities so we have $3.99|S| \leq 5|S|-3f +f$ hence $f \leq 0.505|S|$. Hence using the first lemma we have $|ODS| \geq n-0.505|S|+|S| > n+0.49|S|\geq n+0.49\alpha n$ which violates the approximation ratio at time $t_f$ as dominating set at any time point is less than or equal to $n$. 
\end{proof}





==> SAS_in_graph_class_with_strongly_sublinear_separators.tex <==
\section{Separate and Iterate}
A balanced \emph{separator} $S \subseteq V(G)$ of a graph $G$ with $n$ vertices is a set of vertices removal of which divides the graph into distinct connected components $A$ and $B$ with $|A|\leq 2n/3$ and $|B|\leq 2n/3$. 
In the previous section we have seen that when an online sequence of graphs has expander like property it is not possible to get SAS. Also it is known that expander graphs has linear separators. We observe that the size of separators of the online graphs play an important role in maintaining a SAS. Let $\cg^s$ be a subgraph closed class of graphs such that a graph $G\in \cg^s$ iff it admits a balanced separator of size $c|G|^\delta$ with $\delta<1$. We call the class of graphs $\cg$ as the class of graphs which admits a strongly sublinear separator. In this section we prove  a complimentary result in the sense that if all the dynamic graphs along with all it's subgraphs has strongly sublinear separators then we have SAS. 

Before we prove results on $SAS$ we will prove our main theorem which will show that bipartite graphs with one partition bigger by a factor of the other partition in the class of $\cg$ does not have expander like property even in the weakest sense. We state the precise theorem below which is quite fundamental in nature and might be of independent interest.

\begin{theorem}\label{thm:contraction}
Let $\eps>0$. Let $G_0=I_0 \cup J_0 \in \cg^s$ be a bipartite graph with $I_0$ be the left partition and $J_0$ be the right partition of $G$. Assume $|J_0| > (1+\eps)|I_0|$. Then there exists a constant $k_\eps$ only depending on $\eps$ and not on the size of the graph and a subset $J^* \subseteq J_0$ with $|J^*| \leq k_\eps$ such that $|N(J^*)|<|J^*|$.
\end{theorem}



Before we go to the proof of our theorem we describe the algorithm \textsc{Separate and Iterate} which is presented below. The algorithm takes as input, the bipartite graph $G_0=I_0 \cup J_0 \in \cg^s$ with $I_0$ be the left partition and $J_0$ be the right partition of $G$ and $|J_0| > (1+\eps)|I_0|$. It also takes the appropriate constant $k_\eps$ as stated in theorem \ref{thm:contraction}. The algorithm will output the set $J^* \subseteq J_0$ with the desired property that $|N(J^*)|<|J^*|$ as stated in theorem \ref{thm:contraction}.


\begin{algorithm}[H] 
\caption{\textsc{Separate and Iterate}$(G_k=I_k \cup J_k,k_\eps)$}
\begin{algorithmic}[1]
%
\State $\rhd$ Let $r_k=|J_k|/|I_k|$
\If{$|I_k|+|J_k| \leq k_\eps$}
\State $J^*=J_k$ and output $J^*$.
\Else

    
      \State Find a balanced separator $S_k$ of $G_k$ that separates the graph into two parts $A$ and $B$. Let $I_k \cap A=I_{k,A}$, $J_k \cap A=J_{k,A}$,  $I_k \cap B=I_{k,B}$,  $J_k \cap B=J_{k,B},  I_k \cap S_k=I_{k,S_k},  J_k \cap S_k=J_{k,S_k}$. 
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} < min(1+\eps, r_k)$ and $\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} < min(1+\eps, r_k)$} 
      \State  \textsc{Separate and Iterate}$(G^A,k_\eps)$ where $G^A$ is the induced bipartite subgraph of $G$ with vertices $J_{k,A} \cup I_{k,A} \cup I_{k,S_k}$. 
      \EndIf
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} \geq min(1+\eps, r_k)$}
      \State \textsc{Separate and Iterate}$(G^A,k_\eps)$
        \EndIf
      \If{$\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} \geq min(1+\eps, r_k)$}
      \State \textsc{Separate and Iterate}$(G^B,k_\eps)$ where $G^B$ be the induced bipartite subgraph of $G$ with vertices $J_{k,B} \cup I_{k,B} \cup I_{k,S_k}$.
     
      
      \EndIf
\EndIf
\end{algorithmic}
\end{algorithm}

The algorithm described above is recursive in nature. Once we input the initial graph $G_0$, the algorithm recurses on its own on a finite sequence of bipartite graphs say $G_1=(I_1 \cup J_1), G_2=(I_2 \cup J_2), G_3=(I_3 \cup J_3), \ldots , G_{p+1}=(I_{p+1} \cup J_{p+1})$, before it outputs the desired set $J^*=J_{p+1}$. Assume $n_t=|I_t|+|J_t|$, $r_t=|I_t|/|J_t|$.

Let $G_0=G_{i_0}, G_{i_1}, G_{i_2}, \ldots , G_{i_{q+1}}$ be the largest subset of $G_0, G_1, G_2, G_3, \ldots , G_{p+1}$ containing $G_0$ such that $i_{t+1}=\min \left(i: r_i<r_{i_{t}}, \: i>i_{t}\right)$. This implies that $r_i \geq r_{i_{q+1}}$ for all $i_{q+1}<i\leq p+1$. So all we need to prove is that $r_{i_{q+1}}>1$ as then we have $r_{p+1}>1$, so clearly $|N(J_{p+1})|<|J_{p+1}|$ and we also know that cardinality of $G_{p+1}<k_\eps$, hence we can take $J^*=J_{p+1}$ which will prove our theorem. We will prove the following lemma below before we proceed to the proof of the main theorem. For simplifying the notations let $i_{t+1}-1=i'_t$ for all $t=0, 1, 2, 3, \ldots, q$.

\begin{lemma} \label{lemma:lower bounds of ratios}
Suppose $k_\eps \geq (16c(1+\eps))^{\frac{1}{1-\delta}}$. Then $r_{i_{t+1}}\geq r_{i_t}-\frac{c'}{n_{i'_{t}}}$ for all $t=0, 1, 2, \ldots, q$, where $c'$ is some constant only dependent on $\eps$.
\end{lemma}
\begin{proof} Observe that $r_{i_{t+1}}=|J_{i'_t, A}|/(|I_{i'_t, A}| + |I_{i'_t, S}|)$. From the algorithm we have $k_\eps \leq n_{i'_t}$ for all $t=0, 1, 2, \ldots, q$. By conditions of theorem \ref{thm:contraction} we also have 
$$S_{i'_t} \leq c(n_{i'_t})^{\delta}, |I_{i'_t, A}|+|J_{i'_t, A}| \leq \frac{2n_{i'_t}}{3} \: \text{and} \: |I_{i'_t, B}|+|J_{i'_t, B}| \leq \frac{2n_{i'_t}}{3}$$.
Now since $k_\eps \geq (16c(1+\eps))^{\frac{1}{1-\delta}}$, we have $$n_{i'_t}\geq k_{\eps} \implies n_{i'_t} \geq 16c(1+\eps)(n_{i'_t})^{\delta}=16(1+\eps)|S_{i'_t}| \geq 16(1+\eps)|I_{i'_t, S}|$$. 
So we have $|I_{i'_t, S}| \leq |S_{i'_t}|\leq n_{i'_t}/16(1+\eps)$. We also have $|I_{i'_t, B}|+|J_{i'_t, B}| \leq 2n_{i'_t}/3$, so  $|I_{i'_t, A}|+|J_{i'_t, A}| + |S_{i'_t}| \geq n_{i'_t}/3$. Putting the upper bound of $|S_{i'_t}|$ it is easy to show 
$$|I_{i'_t, A}|+|J_{i'_t, A}| \geq \frac{n_{i'_t}}{4} \: \text{for all} \: t=0, 1, 2, \ldots, q$$
We also have $r_{i_{t+1}}=|J_{i'_t, A}|/(|I_{i'_t, A}|+|I_{i'_t, S}|) \leq 1+\eps$ and together with $|I_{i'_t, A}|+|J_{i'_t, A}| \geq n_{i'_t}/4$ and $|S_{i'_t}|\leq n_{i'_t}/16(1+\eps)$, we get
$$|I_{i'_t, A}|\geq \frac{n_{i'_t}}{16(1+\eps)} \: \text{for all} \: t=0, 1, 2, \ldots, q$$.

Also since $i_{t+1}=\min \left(i: r_i<r_{i_{t}}, \: i>i_{t}\right)$
\begin{flushleft}
$$\frac{|J_{i'_t, A}|}{|I_{i'_t, A}|+|I_{i'_t, S}|}<r_{i'_t} \; \text{and} \; \frac{|J_{i'_t, B}|}{|I_{i'_t, B}|+|I_{i'_t, S}|} < r_{i'_t} \; \forall t=0, 1, 2, \ldots, q \implies |J_{i'_t, B}| \leq r_{i'_t}(|I_{i'_t, B}|+|I_{i'_t, S}|)$$ 

$$\implies \frac{|J_{i'_t, A}|+|J_{i'_t, S}|+ r_{i'_t}(|I_{i'_t, B}|+|I_{i'_t, S}|)}{|I_{i'_t, A}|+ |I_{i'_t, S}|+|I_{i'_t, B}|} \geq r_{i'_t} \implies \frac{|J_{i'_t, A}|+|J_{i'_t, S}|}{|I_{i'_t, A}|} \geq r_{i'_t}   $$
$$\implies |J_{i'_t, A}| \geq r_{i'_t}|I_{i'_t, A}|-|J_{i'_t, S}| \implies r_{i_{t+1}}=\frac{|J_{i'_t, A}|}{|I_{i'_t, A}|+|I_{i'_t, S}|} \geq \frac{r_{i'_t}|I_{i'_t, A}|}{|I_{i'_t, A}|+ |I_{i'_t, S}|}-\frac{|J_{i'_t, S}|}{|I_{i'_t, A}|+ |I_{i'_t, S}|}$$

$$\implies r_{i_{t+1}} \geq \frac{r_{i'_t}|I_{i'_t, A}|}{|I_{i'_t, A}|+ c_2|I_{i'_t, A}|^\delta}-\frac{c(n_{i'_t})^\delta}{|I_{i'_t, A}|} \geq  \frac{r_{i'_t}|I_{i'_t, A}|^{(1-\delta)}}{|I_{i'_t, A}|^{(1-\delta)}+ c_2}-\frac{c_1}{|I_{i'_t, A}|^{(1-\delta)}}$$

Note that $c_1$ and $c_2$ are positive constants. Let $c_3=(1+\eps)c_2+c_1$.\\
\emph{Case 1:\; $r_{i'_t}\leq 1+\eps$}
$$r_{i_{t+1}} \geq \frac{r_{i'_t}|I_{i'_t, A}|^{(1-\delta)}}{|I_{i'_t, A}|^{(1-\delta)}+ c_2}-\frac{c_1}{|I_{i'_t, A}|^{(1-\delta)}} \geq r_{i'_t}- \frac{c_3}{|I_{i'_t, A}|^{1-\delta}}\geq r_{i'_t}- \frac{c'}{(n_{i'_t})^{1-\delta}} $$

\emph{Case 2:\; $r_{i'_t} > 1+\eps$}
$$r_{i_{t+1}} \geq \frac{r_{i'_t}|I_{i'_t, A}|^{(1-\delta)}}{|I_{i'_t, A}|^{(1-\delta)}+ c_2}-\frac{c_1}{|I_{i'_t, A}|^{(1-\delta)}} \geq \frac{(1+\eps)|I_{i'_t, A}|^{(1-\delta)}}{|I_{i'_t, A}|^{(1-\delta)}+ c_2}-\frac{c_1}{|I_{i'_t, A}|^{(1-\delta)}} \geq 1+\eps- \frac{c_3}{|I_{i'_t, A}|^{1-\delta}}\geq 1+\eps- \frac{c'}{(n_{i'_t})^{1-\delta}} $$

Note that in the above two cases $c'$ is a fixed constant. Now since $r_{i_t}\leq \min \left(1+\eps, r_{i'_t}\right)$, we have
$$r_{i_{t+1}} \geq r_{i_t}- \frac{c'}{(n_{i'_{t}})^{1-\delta}} $$

\end{flushleft}
\end{proof}

Now we are ready to prove theorem \ref{thm:contraction} which is given below. Note that in the proof of theorem \ref{thm:contraction} we are implicitly assuming there is already a constant $k_\eps$ without mentioning what is value should be which will be clear only at the end of the proof.

\begin{proof}
\begin{flushleft}
Suppose $k_\eps \geq (16c(1+\eps))^{\frac{1}{1-\delta}}$. As $n_{i'_t}\geq k_\eps$ for all  $t=0, 1, 2, \ldots, q$, we have,
$$n_{i_{t+1}}=|J_{i'_t, A}| + |I_{i'_t, A}| + |I_{i'_t, S}| \leq \frac{2n_{i'_t}}{3} + |I_{i'_t, S}| \leq \frac{2n_{i'_t}}{3} + c(n_{i'_t})^\delta \leq \frac{3n_{i'_t}}{4} \; \text{for all} \; t=0, 1, 2, \ldots, q$$

So we have,
$$n_{i'_{t+1}}\leq n_{i_{t+1}} \leq \frac{3}{4}n_{i'_t} \; \text{for all} \; t=0, 1, 2, \ldots, q$$.
We define the finite sequence $$n_{i_0}=m_0,  \frac{3}{4}n_{i_0}=m_1, \left(\frac{3}{4}\right)^2n_{i_0}=m_2, \ldots, \left(\frac{3}{4}\right)^sn_{i_0}=m_s, \left(\frac{3}{4}\right)^{s+1}n_{i_0}=m_{s+1}$$.

We choose $s$ such that $m_{s+1}\leq k_\eps <m_s$. We know that $k_\eps<n_{i'_q}$. So we have $$m_{s+1}<n_{i'_q} \implies \left(\frac{3}{4}\right)^{s+1}n_{i_0}<n_{i'_q}<n_{i_q}< \left(\frac{3}{4}\right)n_{i'_{q-1}} \implies \left(\frac{3}{4}\right)^{s}n_{i_0}<n_{i'_{q-1}} $$

Continuing the chain of inequalities we have 
$$\left(\frac{3}{4}\right)^{s-x+1}n_{i_0}<n_{i'_{q-x}} \; \text{for all} \; x=0, 1, 2, \ldots q$$

So clearly ,


$$ c'\sum_{t=0}^{q} \frac{1}{(n_{i'_t})^{1-\delta}} \leq c'\sum_{t=s-q+1}^{s+1} \frac{1}{\left((\frac{3}{4})^{t}n_{i_0}\right)^{1-\delta}} \leq c'\sum_{t=0}^{s+1} \frac{1}{\left((\frac{3}{4})^{t}n_{i_0}\right)^{1-\delta}} \leq  \frac{c'}{(n_{i_0})^{1-\delta}}\sum_{t=0}^{s+1} \left(\frac{4^{1-\delta}}{3^{1-\delta}}\right)^t $$

$$\implies c'\sum_{t=0}^{q} \frac{1}{(n_{i'_t})^{1-\delta}} \leq \frac{c'}{(n_{i_0})^{1-\delta}}\left[\frac{\left( (\frac{4}{3})^{1-\delta}\right)^{s+2}-1}{\left( (\frac{4}{3})^{1-\delta}\right)-1}\right]$$


Since $$m_s=\left(\frac{3}{4}\right)^sn_{i_0} > k_\eps \implies \left(\frac{4}{3}\right)^s < \frac{n_{i_0}}{k_\eps}\implies \left( \left(\frac{4}{3}\right)^{1-\delta}\right)^{s+2} <\left(\frac{16}{9}\right)^{1-\delta}\left(\frac{n_{i_0}}{k_\eps}\right)^{1-\delta}$$

So for some constant $c''$ and $k_{\eps} \geq \left(\frac{2c''}{\eps}\right)^{\frac{1}{1-\delta}}$, we have 
$$ c'\sum_{t=0}^{q} \frac{1}{(n_{i'_t})^{1-\delta}} \leq \frac{c''}{(k_\eps)^{1-\delta}} \leq \frac{\eps}{2}$$.

So by taking $k_\eps \geq \max \left(\left(\frac{2c''}{\eps}\right)^{\frac{1}{1-\delta}},\left(16c\right)^{\frac{1}{1-\delta}}\right)$ and combined with lemma \ref{lemma:lower bounds of ratios} we have, 

$$r_{p+1} \geq r_{i_{q+1}} \geq r_{i_0}- c'\sum_{t=0}^{q} \frac{1}{(n_{i'_t})^{1-\delta}}\geq 1+\eps-\frac{\eps}{2} > 1$$

Hence we have our theorem.


\end{flushleft}








\end{proof}


==> mayneed.tex <==
\section{Separate and Iterate Final}
A balanced \emph{separator} $S \subseteq V(G)$ of a graph $G$ with $n$ vertices is a set of vertices removal of which divides the graph into distinct connected components $A$ and $B$ with $|A|\leq 2n/3$ and $|B|\leq 2n/3$. 
In the previous section we have seen that when an online sequence of graphs has expander like property it is not possible to get SAS. Also it is known that expander graphs has linear separators. We observe that the size of separators of the online graphs play an important role in maintaining a SAS. Let $\cg^s$ be a subgraph closed class of graphs such that a graph $G\in \cg^s$ iff it admits a balanced separator of size $c|G|^\delta$ with $\delta<1$. We call the class of graphs $\cg$ as the class of graphs which admits a strongly sublinear separator. In this section we prove  a complimentary result in the sense that if all the dynamic graphs along with all it's subgraphs has strongly sublinear separators then we have SAS. Before we prove our main theorem we describe an algorithm that we will use to prove our main result. Algorithm \textsc{Separate and Iterate} is presented below which takes an input bipartite graph $G=I_k \cup J_k$ where $I_k$ is the left partition and $J_k$ is the right partition with $|J_k|/|I_k|>1$ and also takes a constant $k_\eps $ as input.

\begin{algorithm}[H] 
\caption{\textsc{Separate and Iterate}$(G_k=I_k \cup J_k,k_\eps)$}
\begin{algorithmic}[1]
%
\State $\rhd$ Let $r_k=|J_k|/|I_k|$
\If{$|I_k|+|J_k| \leq k_\eps$}
\State return 1 and terminate.
\Else

    
      \State Find a separator $S_k$ of $G_k$ that separates the graph into two parts $A$ and $B$. Let $I_k \cap A=I_{k,A}$, $J_k \cap A=J_{k,A}$,  $I_k \cap B=I_{k,B}$,  $J_k \cap B=J_{k,B},  I_k \cap S_k=I_{k,S_k},  J_k \cap S_k=J_{k,S_k}$. 
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} < min(1+\eps, 5/4, r_k)$ and $\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} < min(1+\eps, 5/4, r_k)$} 
      \State Output the induced bipartite subgraph $G^A$ of $G$ with vertices $J_{k,A} \cup I_{k,A} \cup I_{k,S_k}$. Then terminate.
      \EndIf
      \If{$\frac{|J_{k,A}|}{|I_{k,A}|+|I_{k,S_k}|} \geq min(1+\eps, 5/4, r_k)$}
      \State Repeat from beginning with new input graph $G=G^A$.
        \EndIf
      \If{$\frac{|J_{k,B}|}{|I_{k,B}|+|I_{k,S_k}|} \geq min(1+\eps, 5/4, r_k)$}
      \State Let $G^B$ be the induced bipartite subgraph of $G$ with vertices $J_{k,B} \cup I_{k,B} \cup I_{k,S_k}$. Repeat from beginning with new input graph $G=G^B$.
     
      
      \EndIf
\EndIf
\end{algorithmic}
\end{algorithm}







\begin{theorem}
Let $\eps>0$. Let $G_0=I_0 \cup J_0 \in \cg^s$ be a bipartite graph with $I_0$ be the left partition and $J_0$ be the right partition of $G$. Assume $|J_0| > (1+\eps)|I_0|$. Then there exists a constant $k_\eps$ and a subset $J^* \subseteq J_0$ with $|J^*| \leq k_\eps$ such that $|N(J^*)|<|J^*|$.
\end{theorem}
\begin{proof}
We assume that there is a constant $k_{\eps}$ large enough, we will give it's exact value in the end, thus proving it's existence and the correctness of the proof will follow. \arp{maybe we can start with the value of $k_\eps$}. We run Algorithm \textsc{Separate and Iterate} repeatedly starting with the intial graph $G_0$ to get a sequence of bipartite graphs $G_1=(I_1 \cup J_1), G_2=(I_2 \cup J_2), G_3=(I_3 \cup J_3), \ldots , G_{p+1}=(I_{p+1} \cup J_{p+1})$. Here $G_t$ is the output graph of the algorithm \textsc{Separate and Iterate} when we input $G_{t-1}$ for all $t=1, 2, \ldots, p+1$. It is easy to see that the algorithm will return $1$ if we recursively input the graphs as the size of the output graphs is strictly less than the input graph. Also note that once we input a graph $G_t$ to the algorithm \textsc{Separate and Iterate}, it may run a few times on it's own and generate a few intermediate graphs before it finally outputs a graph. Let $G_{t'}$ be the last intermediate graph formed by the algorithm when we input $G_t$. Note that we assume that the algorithm \textsc{Separate and Iterate} returns $1$ after we input $G_{p+1}$ to it but does not output $1$ till the input of the graph $G_p$. So if we prove $r_{p+1}>1$ then we are done as then our required set $J^*$ will be equal to $J_{p+1,(p+1)'}$. Let $n_t=|I_t|+|J_t|$, $r_t=|I_t|/|J_t|$, observe that $r_{t+1}=|J_{t',A}|/(|I_{t',A}| + |I_{t',S}|)$. Observe that $k_\eps \leq n_{t'} \leq n_t$ for all $t=1, 2, \ldots, p$. By conditions of the theorem we also have $S_{t'} \leq c(n_t')^{\delta}$, $|I_{t',A}|+|J_{t',A}| \leq 2n_{t'}/3$ and $|I_{t',B}|+|J_{t',B}| \leq 2n_{t'}/3$. Also assume $k_\eps \geq (16c)^{\frac{1}{1-\delta}}$ which implies $n_{t'}\geq 16c(n_{t'})^{\delta}=16|S_{t'}| \geq 16|I_{t',S}|$. Then it is easy to show $|I_{t',A}|+|J_{t',A}| \geq n_t/4$ and also since $|J_{t',A}|/(|I_{t',A}|+|I_{t',S}|) \leq 5/4$, we have $|I_{t',A}|\geq n_{t'}/16$ for all $t=1, 2, \ldots, p$. We also have 
\begin{flushleft}


$$\frac{|J_{t',A}|}{|I_{t',A}|+|I_{t',S}|}<r_{t} \: \text{and} \: \frac{|J_{t',B}|}{|I_{t',B}|+|I_{t',S}|} < r_{t} \: \forall t=0, 1, 2, \ldots, p \implies |J_{t',B}| \leq r_{t}(|I_{t',B}|+|I_{t',S}|)$$ 
$$\implies \frac{|J_{t',A}|+|J_{t',S}|+ r_{t}(|I_{t',B}|+|I_{t',S}|)}{|I_{t',A}|+ |I_{t',S}|+|I_{t',B}|} \geq r_{t} \implies \frac{|J_{t',A}|+|J_{t',S}|}{|I_{t',A}|} \geq r_{t}   $$
$$\implies |J_{t',A}| \geq r_{t}|I_{t',A}|-|J_{t',S}| \implies r_{t+1}=\frac{|J_{t',A}|}{|I_{t',A}|+|I_{t',s}|} \geq \frac{r_{t}|I_{t',A}|}{|I_{t',A}|+ |I_{t',S}|}-\frac{|J_{t',S}|}{|I_{t',A}|+ |I_{t',S}|}$$

$$\implies r_{t+1} \geq \frac{r_{t}|I_{t',A}|}{|I_{t',A}|+ c_2|I_{t',A}|^\delta}-\frac{c(n_{t'})^\delta}{|I_{t',A}|} \geq  \frac{r_{t}|I_{t',A}|^{(1-\delta)}}{|I_{t',A}|^{(1-\delta)}+ c_2}-\frac{c_1}{|I_{t',A}|^{(1-\delta)}}$$

Note that $c_1$ and $c_2$ are positive constants.
Also since $r_{t}$ is bounded by $\min\left((1+\eps),5/4\right)$, by simple calculation it is easy to see that there exist a constant $c_3,c_4>0$ 

$$r_{t+1} \geq r_{t}- \frac{c_3}{|I_{t',A}|^{1-\delta}}\geq r_{t}- \frac{c_4}{(n_t')^{1-\delta}} $$

\arp{pls check the equations below carefully, there may be errors}

It is easy to see $n_{(t+1)'}\leq n_{t+1}\leq \frac{3}{4}n_{t'}$. We define a sequence $n_0=m_0,  (3/4)n_0=m_1, (3/4)^2n_0=m_2, \ldots, (3/4)^sn_0=m_s, (3/4)^{s+1}n_0=m_{s+1}$.

Clearly $s\geq p$. Also assume $m_{s+1}\leq k_\eps <m_s$. We know that $k_\eps<n_{p'}$. So we have $m_{s+1}<n_{p'} \implies (\frac{3}{4})^{s+1}n_0<n_p \leq (\frac{3}{4})n_{(p-1)'} \implies (\frac{3}{4})^{s}n_0<n_{(p-1)'}\implies (\frac{3}{4})^{s-x+1}n_0<n_{(p-x)'} $



So clearly ,


$$ c_4\sum_{t=0}^{p} \frac{1}{(n_{t'})^{1-\delta}} \leq c_4\sum_{t=0}^{s+1} \frac{1}{((\frac{3}{4})^{t}n_0)^{1-\delta}}\leq  \frac{c_4}{(n_0)^{1-\delta}}\sum_{t=0}^{s+1} \left(\frac{4^{1-\delta}}{3^{1-\delta}}\right)^t $$

$$\implies \frac{c_4}{(n_0)^{1-\delta}}\sum_{t=0}^{s+1} \left(\frac{4^{1-\delta}}{3^{1-\delta}}\right)^t= \frac{c_4}{(n_0)^{1-\delta}}\left[\frac{\left( (\frac{4}{3})^{1-\delta}\right)^{s+2}-1}{\left( (\frac{4}{3})^{1-\delta}\right)-1}\right]$$


Since $$m_s=\left(\frac{3}{4}\right)^sn_0 > k_\eps \implies \left(\frac{4}{3}\right)^s < \frac{n_0}{k_\eps}\implies \left( \left(\frac{4}{3}\right)^{1-\delta}\right)^{s+2} <c_6\left(\frac{n_0}{k_\eps}\right)^{1-\delta}$$

So for some constants $c_7$ and $c_8$ and $k_{\eps} \geq \left(\frac{2c_7}{\eps}\right)^{\frac{1}{1-\delta}}$, we have 
$$ c_4\sum_{t=0}^{p} \frac{1}{(n_{t'})^{1-\delta}} \leq \frac{c_7}{(k_\eps)^{1-\delta}}-\frac{1}{c_8(n_0)^{1-\delta}} \leq \frac{\eps}{2}$$.

So by taking $k_\eps \geq \max \left(\left(\frac{2c_7}{\eps}\right)^{\frac{1}{1-\delta}},\left(16c\right)^{\frac{1}{1-\delta}}\right)$ we have, 

$$r_{p+1}=r_0- c_4\sum_{t=0}^{p} \frac{1}{(n_{t'})^{1-\delta}}\geq 1+\eps-\frac{\eps}{2} > 1$$


\end{flushleft}








\end{proof}

